Grounding Text-to-Image Diffusion Models for Controlled High-Quality Image Generation

Text-to-image (T2I) generative diffusion models have demonstrated outstanding performance in synthesizing diverse, high-quality visuals from text captions. Several layout-to-image models have been developed to control the generation process by utilizing a wide range of layouts, such as segmentation maps, edges, and human keypoints. In this work, we propose ObjectDiffusion, a model that conditions T2I diffusion models on semantic and spatial grounding information, enabling the precise rendering and placement of desired objects in specific locations defined by bounding boxes. To achieve this, we make substantial modifications to the network architecture introduced in ControlNet to integrate it with the grounding method proposed in GLIGEN. We fine-tune ObjectDiffusion on the COCO2017 training dataset and evaluate it on the COCO2017 validation dataset. Our model improves the precision and quality of controllable image generation, achieving an AP$_{\text{50}}$ of 46.6, an AR of 44.5, and an FID of 19.8, outperforming the current SOTA model trained on open-source datasets across all three metrics. ObjectDiffusion demonstrates a distinctive capability in synthesizing diverse, high-quality, high-fidelity images that seamlessly conform to the semantic and spatial control layout. Evaluated in qualitative and quantitative tests, ObjectDiffusion exhibits remarkable grounding capabilities in closed-set and open-set vocabulary settings across a wide variety of contexts. The qualitative assessment verifies the ability of ObjectDiffusion to generate multiple detailed objects in varying sizes, forms, and locations.

==> Makefile <==
main:
	pdflatex main

full:
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main

camready: full
	gs -dNOPAUSE -dBATCH -dNOPLATFONTS -sDEVICE=pdfwrite -dEmbedAllFonts=true -sOutputFile=main-gs.pdf -f main.pdf

cut: full
	pdftk main.pdf cat 1-11 output main_submit.pdf
	pdftk main.pdf cat 12-end 9-11 output suppl_submit.pdf

clean:
	rm *.aux *.bbl *.blg *.log *.pdf *.dep *.brf *.fls *.out

run:
	evince main.pdf

compress:
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/default -dNOPAUSE -dQUIET -dBATCH -dDetectDuplicateImages -dCompressFonts=true -r150 -sOutputFile=suppl.pdf suppl_highRes.pdf

arxiv: full
	rm -rf ../arxiv.tar.gz ../paper_arXiv
	cd ../arxiv-latex-cleaner && python3.9 -m arxiv_latex_cleaner ../paper/
	# Unfortunately it still doesn't remove unused PDF etc files... need to use the arxiv-collector
	rm -f /tmp/latexmk
	cd .. && python3.9 arxiv-collector/arxiv_collector.py --get-latexmk /tmp/latexmk
	cd ../paper_arXiv && python3.9 ../arxiv-collector/arxiv_collector.py --latexmk /tmp/latexmk main.tex
	mv ../paper_arXiv/arxiv.tar.gz ../
	rm -rf ../paper_arXiv


